JaSPICE: Automatic Evaluation Metric Using Predicate-Argument Structures for Image Captioning Models

Image captioning studies heavily rely on automatic evaluation metrics such as BLEU and METEOR. However, such n-gram-based metrics have been shown to correlate poorly with human evaluation, leading to the proposal of alternative metrics such as SPICE for English; however, no equivalent metrics have been established for other languages. Therefore, in this study, we propose an automatic evaluation metric called JaSPICE, which evaluates Japanese captions based on scene graphs. The proposed method generates a scene graph from dependencies and the predicate-argument structure, and extends the graph using synonyms. We conducted experiments employing 10 image captioning models trained on STAIR Captions and PFN-PIC and constructed the Shichimi dataset, which contains 103,170 human evaluations. The results showed that our metric outperformed the baseline metrics for the correlation coefficient with the human evaluation.

==> section7.tex <==
% \vspace{-1mm}
% \section{Conclusions}
% \vspace{-1mm}
% In this paper we proposed JaSPICE, an automatic evaluation metric for image captioning models in Japanese.
% The following contributions of this study can be emphasized:
% \begin{itemize}
%     \item We proposed JaSPICE, an automatic evaluation metric for image captioning models in Japanese.
%     \item Unlike SPICE, we proposed a rule-based scene graph parser PAS-SGP using dependencies and PAS.
%     \item We introduced graph expansion using synonyms to take synonyms into account in the evaluation.
%     \item Our method outperformed SPICE calculated from English translations and the baseline metrics on the correlation coefficient with the human evaluation.
% \end{itemize}

% Future studies will extend our method by taking into account hypernyms and hyponyms.


==> tab/baseline_comp.tex <==
\begin{table*}[tb]
\centering
%\footnotesize
\caption{
\textbf{Quantitative comparison and ablation studies.}
The methods have been compared on the CoDraw and i-CLEVR datasets according to several metrics:
the average precision~(AP), average recall (AR), F1-score, and relational similarity (RSIM).
For each metric and dataset, the best scores are in bold,
and the second best ones are underlined.
The mean and standard deviation have been calculated on five different seed runs.
% For i-CLEVR, our model boosted the recall by 12.4 point,
% which resulted in the F1 and RSIM are also improved. 
}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{@{}lccccccccc@{}}
\toprule
           & \multicolumn{4}{c}{CoDraw}            & \multicolumn{1}{l}{} & \multicolumn{4}{c}{i-CLEVR}           \\ \cmidrule(lr){2-5} \cmidrule(l){7-10} 
Methods      & AP$\uparrow$ & AR$\uparrow$ & F1$\uparrow$ & RSIM$\uparrow$  &
& AP$\uparrow$ & AR$\uparrow$ & F1$\uparrow$ & RSIM$\uparrow$  \\ \midrule

% fixed (paper result)
GeNeVA-GAN~{\tiny} & 66.64     & 52.66  & 58.83    & 35.41 &                      & 92.39     & 84.72  & 88.39    & 74.02 \\ \midrule

% fixed (single run, actual results)
% Ours (w/o Latte \& TxtCond)   & 75.33  & 74.05  & 71.98  & 47.13  & & 95.19  & 93.92  & 94.45  & 78.28  \\
Ours (w/o Latte \& TxtCond)
& $76.75{\scriptscriptstyle \pm0.94}$    
& $73.99{\scriptscriptstyle \pm0.11}$ 
& $72.81{\scriptscriptstyle \pm0.51}$
& $47.43{\scriptscriptstyle \pm0.28}$  &
& $95.77{\scriptscriptstyle \pm0.59}$
& $94.60{\scriptscriptstyle \pm0.69}$
& $95.08{\scriptscriptstyle \pm0.65}$
& $79.31{\scriptscriptstyle \pm1.23}$ \\

% temporal (single run, expected results (+4, -1, +2, +.5, +3.5, +4, +4, +5))
% \txq{w/o Latte}        & 79.33  & 73.05  & 73.98  & 47.63  & & 98.69  & 97.92  & 98.45  & 83.28  \\
% Ours (w/o Latte)              & 77.82  & 73.54  & 73.03  & 47.96  & & \bf{98.91}  & \bf{98.58}  & \bf{98.72}  & \bf{83.95}  \\
Ours (w/o Latte)
& $79.04{\scriptscriptstyle \pm1.28}$    
& $73.91{\scriptscriptstyle \pm0.53}$ 
& $74.02{\scriptscriptstyle \pm1.03}$
& $48.16{\scriptscriptstyle \pm0.41}$  &
& $\bm{98.35}{\scriptscriptstyle \pm1.27}$
& $\bm{97.68}{\scriptscriptstyle \pm1.61}$
& $\bm{97.96}{\scriptscriptstyle \pm1.47}$
& $\underline{82.78}{\scriptscriptstyle \pm1.94}$ \\

% fixed (single run, actual results)
% Ours (w/o TxtCond)            & \bf{81.48}  & \bf{78.33}  & \bf{77.51}  & 53.41  & & 96.32  & 95.20  & 95.67  & 80.21  \\
Ours (w/o TxtCond)
& $\underline{80.53}{\scriptscriptstyle \pm0.97}$    
& $\bm{78.42}{\scriptscriptstyle \pm0.38}$ 
& $\underline{77.11}{\scriptscriptstyle \pm0.60}$
& $\underline{53.13}{\scriptscriptstyle \pm0.25}$  &
& $96.67{\scriptscriptstyle \pm0.41}$
& $95.52{\scriptscriptstyle \pm0.43}$
& $95.99{\scriptscriptstyle \pm0.42}$
& $81.04{\scriptscriptstyle \pm0.97}$ \\

% temporal (multiple run, expected results (+4, -1, +2, +.5, +3.5, +4, +4, +5))
% \txq{\bf{LatteGAN (Ours)}}
% & ${85.48}{\scriptscriptstyle \pm0.00}$    
% & ${77.33}{\scriptscriptstyle \pm0.00}$ 
% & ${79.51}{\scriptscriptstyle \pm0.00}$
% & ${53.91}{\scriptscriptstyle \pm0.00}$  &
% & ${99.82}{\scriptscriptstyle \pm0.00}$
% & ${99.20}{\scriptscriptstyle \pm0.00}$
% & ${99.67}{\scriptscriptstyle \pm0.00}$
% & ${85.21}{\scriptscriptstyle \pm0.00}$ \\ \bottomrule
\bf{Ours (LatteGAN)}
& $\bm{81.50}{\scriptscriptstyle \pm0.82}$    
& $\underline{78.37}{\scriptscriptstyle \pm0.38}$ 
& $\bm{77.51}{\scriptscriptstyle \pm0.52}$
& $\bm{54.16}{\scriptscriptstyle \pm0.21}$  &
& $\underline{97.72}{\scriptscriptstyle \pm1.44}$
& $\underline{96.93}{\scriptscriptstyle \pm1.64}$
& $\underline{97.26}{\scriptscriptstyle \pm1.56}$
& $\bm{83.21}{\scriptscriptstyle \pm1.70}$ \\ \bottomrule

\end{tabular}
\end{adjustbox}
\label{tab:results}
\end{table*}

==> tab/params.tex <==

\begin{table}[t]
    \centering
    % \vspace{-6mm}
    \caption{\small Parameter settings of the ABEN}
    \vspace{-2mm}
    \small
    \begin{tabular}{|c|l|}
        \hline
         Opt. & Adam ( Learning rate $=1.0 \times 10^{-4},$ \\
         method & $\beta_1=0.7, \beta_2=0.99999$ ) \\ \hline
        Backbone CNN &  ResNet-50 \\ \hline
        % Embedded vector size &  768 \\ \hline
        LSTM & 3 layers, 768-dimensional cell \\ \hline
        $N$ & 10 \\ \hline
        Generation Branch & FC: 768, 768 \\ \hline
        % MLP num. nodes &  [768, 768] \\ \hline
        % input N size &  downscaled to $(224 \times 224 \times 3)$ \\ \hline
        Batch size & 32 \\ \hline
    \end{tabular}
    \label{tab:parameters}
    \vspace{-6mm}
\end{table}


